Metric Dimension Parameterized by Feedback Vertex Set and Other Structural Parameters

For a graph $G$, a subset $S \subseteq V(G)$ is called a \emph{resolving set} if for any two vertices $u,v \in V(G)$, there exists a vertex $w \in S$ such that $d(w,u) \neq d(w,v)$. The {\sc Metric Dimension} problem takes as input a graph $G$ and a positive integer $k$, and asks whether there exists a resolving set of size at most $k$. This problem was introduced in the 1970s and is known to be \NP-hard~[GT~61 in Garey and Johnson's book]. In the realm of parameterized complexity, Hartung and Nichterlein~[CCC~2013] proved that the problem is \W[2]-hard when parameterized by the natural parameter $k$. They also observed that it is \FPT\ when parameterized by the vertex cover number and asked about its complexity under \emph{smaller} parameters, in particular the feedback vertex set number. We answer this question by proving that {\sc Metric Dimension} is \W[1]-hard when parameterized by the combined parameter feedback vertex set number plus pathwidth. This also improves the result of Bonnet and Purohit~[IPEC 2019] which states that the problem is \W[1]-hard parameterized by the pathwidth. On the positive side, we show that {\sc Metric Dimension} is \FPT\ when parameterized by either the distance to cluster or the distance to co-cluster, both of which are smaller parameters than the vertex cover number.

==> dombay_plate_gadget.tex <==
\begin{tikzpicture}
\node[circ,label=below:{\small $g$}] (g) at (6.125,7.5) {};
\node[circ,label=above:{\small $g_1$}] (g1) at (5.625,7.75) {};
\node[circ,label=above:{\small $g_2$}] (g2) at (6.625,7.75) {};


% G_x1
\node[circ,label=left:{\small $t_1$}] (t1) at (0,5.25) {};

\node[circ,label=above:{\small $a^1_1$}] (a11) at (0.5,5.75) {};
\node[circ,label=above:{\small $b^1_1$}] (b11) at (1.25,5.75) {};

\node[circ,label=below:{\small $a^2_1$}] (a12) at (0.5,4.75) {};
\node[circ,label=below:{\small $b^2_1$}] (b12) at (1.25,4.75) {};

\node[circ,label=right:{\small $f_1$}] (f1) at (1.75,5.25) {};

% G_x2
\node[circ,label=left:{\small $t_2$}] (t2) at (3,5.25) {};

\node[circ,label=above:{\small $a^1_2$}] (a21) at (3.5,5.75) {};
\node[circ,label=above:{\small $b^1_2$}] (b21) at (4.25,5.75) {};

\node[circ,label=below:{\small $a^2_2$}] (a22) at (3.5,4.75) {};
\node[circ,label=below:{\small $b^2_2$}] (b22) at (4.25,4.75) {};

\node[circ,label=right:{\small $f_2$}] (f2) at (4.75,5.25) {};

\node[draw=none] at (5.75,5.25) {$\cdots$};

\node[circ,label=left:{\small $t_i$}] (ti) at (6.75,5.25) {};

\node[circ,label=above:{\small $a^1_i$}] (ai1) at (7.25,5.75) {};
\node[circ,label=above:{\small $b^1_i$}] (bi1) at (8,5.75) {};

\node[circ,label=below:{\small $a^2_i$}] (ai2) at (7.25,4.75) {};
\node[circ,label=below:{\small $b^2_i$}] (bi2) at (8,4.75) {};

\node[circ,label=right:{\small $f_i$}] (fi) at (8.5,5.25) {};

\node[draw=none] at (9.5,5.25) {$\cdots$};

\node[circ,label=left:{\small $t_n$}] (tn) at (10.5,5.25) {};

\node[circ,label=above:{\small $a^1_n$}] (an1) at (11,5.75) {};
\node[circ,label=above:{\small $b^1_n$}] (bn1) at (11.75,5.75) {};

\node[circ,label=below:{\small $a^2_n$}] (an2) at (11,4.75) {};
\node[circ,label=below:{\small $b^2_n$}] (bn2) at (11.75,4.75) {};

\node[circ,label=right:{\small $f_n$}] (fn) at (12.25,5.25) {};


\node[draw=none] at (4.25,2.5) {$\cdots$};

\node[circ,label=left:{\small $c^1_j$}] (c1j) at (5.25,2.5) {};
\node[circ,label=right:{\small $c^2_j$}] (c2j) at (7,2.5) {};

\node[draw=none] at (8,2.5) {$\cdots$};

\node[circ,label=left:{\small $z_1$}] (z1) at (3.5,1) {};
\node[circ,label=below:{\small $z^1_1$}] (z11) at (3,.25) {};
\node[circ,label=below:{\small $z^2_1$}] (z12) at (4,.25) {};

\node[circ,label=left:{\small $z_2$}] (z2) at (5,1) {};
\node[circ,label=below:{\small $z^1_2$}] (z21) at (4.5,.25) {};
\node[circ,label=below:{\small $z^2_2$}] (z22) at (5.5,.25) {};

\node[draw=none] at (6,1) {$\cdots$};
\node[circ,label=left:{\small $z_i$}] (zi) at (7, 1) {};
\node[circ,label=below:{\small $z^1_i$}] (zi1) at (6.5,.25) {};
\node[circ,label=below:{\small $z^2_i$}] (zi2) at (7.5,.25) {};

\node[draw=none] at (8,1) {$\cdots$};

\node[circ,label=left:{\small $z_{\alpha}$}] (zn) at (9,1) {};
\node[circ,label=below:{\small $z^1_{\alpha}$}] (zn1) at (8.5,.25) {};
\node[circ,label=below:{\small $z^2_{\alpha}$}] (zn2) at (9.5,.25) {};

\draw (t1) -- (a11)
(t1) -- (a12)
(a11) -- (b11)
(a12) -- (b12)
(b11) -- (f1)
(b12) -- (f1)
(t2) -- (a21)
(t2) -- (a22)
(a21) -- (b21)
(a22) -- (b22)
(b21) -- (f2)
(b22) -- (f2)
(ti) -- (ai1)
(ti) -- (ai2)
(ai1) -- (bi1)
(ai2) -- (bi2)
(bi1) -- (fi)
(bi2) -- (fi)
(tn) -- (an1)
(tn) -- (an2)
(an1) -- (bn1)
(an2) -- (bn2)
(bn1) -- (fn)
(bn2) -- (fn)
(z1) -- (z11)
(z1) -- (z12)
(z2) -- (z21)
(z2) -- (z22)
(zi) -- (zi1)
(zi) -- (zi2)
(zn) -- (zn1)
(zn) -- (zn2)
(g) -- (g1)
(g) -- (g2)
(g) .. controls (0.25,7) .. (t1)
(g) .. controls (12,7) .. (fn)
(g) .. controls (2,6.75) .. (f1)
(g) .. controls (10.25,6.75) .. (tn)
(g) .. controls (3,6.5) .. (t2)
(g) .. controls (4.75,6.25) .. (f2)
(g) .. controls (6.75,6.75) .. (ti)
(g) .. controls (8.5,6.75) .. (fi)

(c2j) .. controls (6.5,4) and (0,2) .. (t1)
(c2j) .. controls (7.25,4) and (12.25,2) .. (fn)
(c2j) .. controls (6.5,4) and (1.75,2.25) .. (f1)
(c2j) .. controls (7.25,4) and (10.5,3) .. (tn)
(c2j) .. controls (6.5,4) and (3,2.5) .. (t2)
(c2j) .. controls (6.5,4) and (5,3.5) .. (f2)
(c2j) .. controls (6.75,4) .. (ti)
(c2j) .. controls (7.25,4) and (8.5,2.75) .. (fi)

(c1j) .. controls (5,3.5) and (0,2) .. (t1)
%(c1j) .. controls (7.25,4.25) and (12.25,2) .. (fn)
%(c1j) .. controls (5,3.25) and (1.75,2.25) .. (f1)
(c1j) .. controls (5.5,3.25) and (10.5,3.75) .. (tn)
%(c1j) .. controls (6.5,4.25) and (3,2.5) .. (t2)
(c1j) .. controls (5,3.5) and (4.75,3.5) .. (f2)
(c1j) .. controls (5.5,3.5) and (6.75,3.75) .. (ti)
(c1j) .. controls (5.5,3.5) and (8.5,3.25) .. (fi);

\begin{scope}[on background layer]
\draw (c1j) -- (z1)
(c1j) -- (z2)
(c1j) -- (zn)
(c1j) -- (zi)
(c2j) -- (z1)
(c2j) -- (z2)
(c2j) -- (zi)
(c2j) -- (zn);
\end{scope}

\draw[draw=black, fill=white] (4,1.5) rectangle ++(4.5,0.5);
\node at (6.25,1.75) {according to bin(j)};

\end{tikzpicture}


==> vertex-cover.tex <==
\section{The Vertex Cover Number and the Distance to clique}\label{sec:nopolykernel}

In this section, we prove that {\sc Metric Dimension} parameterized by either the vertex cover number or the distance to clique does not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$. The two reductions are similar and start from the {\sc SAT} problem, in which we are given a conjunctive normal form (CNF) formula $\phi$ on $n$ variables and $m$ clauses, and we are asked whether there exists an assignment of either true or false to each of the variables, such that $\phi$ is true (satisfied). The {\sc SAT} problem is known to not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$~\cite{FS11}. 
We first prove that {\sc Metric Dimension} parameterized by the vertex cover number does not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$, and then prove the same result for the distance to clique by slightly modifying the latter reduction.

\begin{theorem}\label{polyker}
{\sc Metric Dimension} parameterized by the vertex cover number does not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$.
\end{theorem}

\begin{proof}
By a reduction from {\sc SAT}, we prove that {\sc Metric Dimension} parameterized by the vertex cover number does not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$.
Let $\phi$ be an instance of {\sc SAT}, that is, $\phi$ is a SAT formula on $n$ variables $x_1,\dots,x_n$ and $m$ clauses $C_1,\dots,C_m$.
Since any {\sc SAT} formula on $n$ variables trivially has at most $3^n-1$ unique clauses, 
we may assume that $m\leq 3^n-1$.
From $\phi$, we construct an instance $(G,k)$ of {\sc Metric Dimension} such that the instance $\phi$ is satisfiable if and only if $(G,k)$ is a \yes-instance for {\sc Metric Dimension}.
Set $k=n+\alpha+1$.\\

\noindent
\textbf{Reduction.}
The construction of $G$ is as follows (see Figure~\ref{fig:dombay_plate_gadget} for an illustration).
\begin{itemize}
\item For each $i\in [n]$, construct a cycle $(t_ia_i^1b_i^1f_ib_i^2a_i^2t_i)$ on $6$ vertices, and let $I_i:=\{a_i^1, a_i^2, b_i^1, b_i^2\}$.
\item Construct a path $(g^1gg^2)$ on $3$ vertices and
for each $i\in [n]$, make both $f_i$ and $t_i$ adjacent to $g$.
\item For each $j\in [m]$, add a pair of vertices $c_j^1$ and $c_j^2$, and let $C_j:=\{c_j^1, c_j^2\}$.
\item For each $j\in [m]$, make $c_j^2$ adjacent to both $f_i$ and $t_i$ for each $i\in [n]$. 
\item For each $j\in [m]$ and each $i \in [n]$, if $x_i =\true$ does not satisfy the clause $\mathcal{C}_j$ in $\phi$, then make $c_j^1$ adjacent to $t_i$, and if $x_i=\false$ does not satisfy $\mathcal{C}_j$, then make $c_j^1$ adjacent to $f_i$.
\item Let $\alpha=\lceil n\cdot \log_{2}3\rceil$, and, for each $\ell\in [\alpha]$, construct a path $(z_{\ell}^1z_{\ell}z_{\ell}^2)$ on $3$ vertices.
\item For each $j\in [m]$, consider the binary representation $\bin(j)$ of $j$, and connect both $c_j^1$ and $c_j^2$ with $z_{\ell}$ if $\bin(j)[\ell]=1$, where $[\ell]$ represents the $\ell^{th}$ bit of $j$ in its binary representation going from right to left.
\item Finally, construct a clique on the vertices $z_1,\dots,z_{\alpha},g$.
\end{itemize}
This completes the construction of the graph $G$, which is clearly achieved in polynomial time.
To simplify notation for the proof, let $T:=\{t_1,\dots,t_n\}\cup \{f_1,\dots,f_n\}$ and $I:=I_1\cup \cdots \cup I_n$.

\begin{figure}[t]
\centering
\scalebox{0.7}{
\input{dombay_plate_gadget}
}
\caption{Illustration of the graph $G$ constructed in the proof of Theorem~\ref{polyker}. The vertices $z_1,\dots,z_{\alpha},g$ are in a clique that is not drawn. In this particular case, $\phi$ has a clause $(\overline{x_1}\vee x_2 \vee \overline{x_n})$.}
\label{fig:dombay_plate_gadget}
\end{figure}

\begin{claim}
If $\phi$ is satisfiable then $(G,k)$ is a \yes-instance for {\sc Metric Dimension}.
\end{claim}
\begin{claimproof}
Assume that $\phi$ is satisfiable 
and consider a truth assignment of the variables of $\phi$ satisfying $\phi$.
We construct a resolving set $R$ of $G$ of size at most $k=n+\alpha+1$ as follows.
Let $R_1:=\{g^1,z_1^1,\dots,z_{\alpha}^1\}$ be an ordered subset of vertices.
Let $R_2$ be an initially empty ordered subset of vertices. 
We add vertices to $R_2$ in such a way that 
the $i^{th}$ added vertex is in the $i^{th}$ position of the ordered subset. 
For each $i\in [n]$, if $x_i=\true$ ($x_i=\false$, respectively) in the considered truth assignment, 
then add $a_i^1$ ($b_i^1$, respectively) to $R_2$.
Let $R:=R_1\cup R_2$ be the ordered subset of vertices with the vertices of $R_1$ appearing in order before the vertices of $R_2$ (also in order).

Let us show that $R$ is indeed a resolving set of $G$.
Clearly, the vertices of $R$ distinguish themselves.
According to Table~\ref{partvect}, the vertices of $R_1$ resolve any two vertices $u,v\in V(G)$ except in the following three cases: (1)~$\{u,v\}\subseteq T\cup \{g^2\}$; (2)~$\{u,v\} \subseteq I$ or (3)~$u\in C_j$ and $v\in C_j\cup \{z_1^2,\dots,z_{\alpha}^2\}$ for some $j\in [m]$.
Thus, the remaining $n$ vertices of $R_2$ must resolve $u$ and $v$ in these cases; 
we consider below each case one by one. \\

\begin{table}[ht]
\begin{center}
\begin{tabular}{l|l}
Vertex set $v$ is in &	$r(R_1|v)$\\\hline
$\{g^2\}$	&	$(2,3,\ldots, 3)$\\
$\{g\}$		&	$(1,2,\ldots, 2)$\\
$T$	&	$(2,3,\ldots, 3)$\\
$I$	&	$(3,4,\ldots, 4)$\\
$C_j$ for some $j\in [m]$	&	$(3,3-\bin(j)[i],\ldots,3-\bin(j)[\alpha])$\\
$\{z_{\ell}\}$ for some $\ell\in [\alpha]$	&	$(2,2,\ldots, 2,\underbracket{1}_{i^{\text{th}}},2,\ldots, 2)$\\
$\{z^2_{\ell}\}$ for some $\ell\in [\alpha]$	&	$(3,3,\ldots, 3,\underbracket{2}_{i^{\text{th}}},3,\ldots, 3)$
\end{tabular} 
\caption{Distance vector of $R_1$ with respect to $v$ for different cases of $v\in V(G)$.} 
\label{partvect}
\end{center}
\end{table}

\noindent 
{\bf Case 1.} \emph{$\{u,v\}\subseteq T\cup \{g^2\}$.} 
For each $i\in [n]$, there is a vertex $w_i\in \{a_i^1,b_i^1\}\cap R_2$
and so, $d(w_i,g^2)=3$ and $d(w_i,t_s)=d(w_i,f_s)=3$ for all $s\in [n]$ such that $s\neq i$. 
Moreover, if $w_i=a_i^1$ ($w_i=b_i^1$, respectively), then $d(w_i,t_i)=1$ and $d(w_i,f_i)=2$ ($d(w_i,t_i)=2$ and $d(w_i,f_i)=1$, respectively).
Thus, the vertices $u$ and $v$ are resolved in this case.\\

\noindent 
{\bf Case 2.} \emph{$\{u,v\} \subseteq I$.}
As in the previous case, for each $i\in [n]$, there is a vertex $w_i\in \{a_i^1,b_i^1\}\cap R_2$, and so, $d(w_i,q)=4$ for all $q\in I\setminus I_i$. 
Moreover, if $w_i=a_i^1$ ($w_i=b_i^1$, respectively), then $d(w_i,b_i^1)=1$, $d(w_i,a_i^2)=2$, and $d(w_i,b_i^2)=3$ ($d(w_i,a_i^1)=1$, $d(w_i,b_i^2)=2$, and $d(w_i,a_i^2)=3$, respectively).
Thus, the vertices $u$ and $v$ are resolved in this case.\\

\noindent 
{\bf Case 3.} \emph{$u\in C_j$ and $v\in C_j\cup \{z_1^2,\ldots,z_{\alpha}^2\}$ for some $j\in [m]$.}
Let $s \in [n]$ be such that $x_s$ satisfies clause $C_j$ in the considered truth assignment of the variables.
By construction, there exists $w \in \{a_s^1,b_s^1\}\cap R_2$.
We claim that $d(w,c_j^1)=3$.
Indeed, if $w=a_s^1$ ($w=b_s^1$, respectively) then by construction, setting $x_s$ to \true\ (\false, respectively) satisfies the clause $C_j$ in $\phi$, and hence, there is no edge between $t_s$ ($f_s$, respectively) and $c_j^1$ in $G$.
Note that for all $i\in [n]$, $j\in [m]$, and $\ell \in [\alpha]$, for any vertex $q\in I$, $d(q,c_j^2)=2$ and $d(q,z_{\ell}^2)=4$.
Thus, the vertices $u$ and $v$ are resolved in this case.\\		

Since in every case, the vertices $u$ and $v$ are resolved by $R$, we conclude that $R$ is indeed a resolving set;
and since $|R|=n+\alpha+1$, the claim follows.
\end{claimproof}


\begin{claim}
If $(G,k)$ is a \yes-instance for {\sc Metric Dimension} then $\phi$ is satisfiable.
\end{claim}

\begin{claimproof}
Assume that $(G,k)$ is a \yes-instance for \mdfull\ and let $R$ be a resolving set of size at most $k$.
By \Cref{obs:twins}, $R$ contains at least one vertex in $\{g^1,g^2\}$
and at least one vertex in $\{z_{\ell}^1,z_{\ell}^2\}$ for every $\ell \in [\alpha]$.
Furthermore, since for every $i \in [n]$, $d(a_i^1,t_i)=d(a_i^2,t_i)$, $d(a_i^1,f_i)=d(a_i^2,f_i)$, 
and $t_i$ and $f_i$ separate $I_i$ from the rest of $G$, 
necessarily$R \cap I_i \neq \emptyset$.
Since $|R| \le n+\alpha+1$, this implies, in particular, that $|R \cap \{g^1,g^2\}| = 1$, $|R \cap \{z_{\ell}^1,z_{\ell}^2\}| = 1$ for all $\ell\in [\alpha]$, and $|R \cap I_i| = 1$ for every $i \in [n]$.

Without loss of generality, let us assume that $\{g^1,z_1^1,\dots,z_{\alpha}^1\}\subset R$.
Consider $j \in [m]$.
As shown in \Cref{partvect}, no vertex in $\{g^1,z_1^1,\dots,z_{\alpha}^1\}$ can resolve two vertices of $C_j$, 
and thus, there must exist $w \in R \cap I$ such that $d(w,c^1_j) \neq d(w,c^2_j)$.
Since for every $i \in [n]$ such that $x_i$ does not appear in the clause $C_j$, 
$d(u,c^1_j) = d(u,c^2_j)$ for every $u \in I_i$,
there must exist $i \in [n]$ such that $x_i$ appears in the clause $C_j$ and $w \in R \cap I_i$. 
In particular, $c^1_j$ must be nonadjacent to one of $t_i$ and $f_i$.
Now, if $c^1_j$ is nonadjacent to $t_i$, then, by construction, $c^1_j$ is adjacent to $f_i$, 
and so, $w \in \{a^1_i,a^2_i\}$ as otherwise $d(w,c^1_j) = d(w,c^2_j)$.
Symmetrically, if  $c^1_j$ is nonadjacent to $f_i$, then, by construction, $c^1_j$ is adjacent to $t_i$, 
and so, $w \in \{b^1_i,b^2_i\}$ as otherwise $d(w,c^1_j) = d(w,c^2_j)$.
It follows that the truth assignment obtained by setting a variable $x_i$ to \true\ if $R \cap I_i \subseteq \{a^1_i,a^2_i\}$,
and to \false\ otherwise, satisfies every clause. 
\end{claimproof}

Lastly, note that the vertex cover number of $G$ is at most $4n+\alpha+1$ 
since $\{g\}\cup T\cup \{a_1^1,\dots a_n^1\} \cup \{a_1^2,\dots a_n^2\} \cup \{z_1,\dots,z_{\alpha}\}$ 
is a vertex cover of $G$. 
Hence, the existence of a polynomial kernel for {\sc Metric Dimension} parameterized by the vertex cover number of $G$ would contradict the fact that there is no polynomial kernel for {\sc SAT} parameterized by the number of its variables,
which concludes the proof.
\end{proof}

\begin{theorem}\label{clique_polyker}
{\sc Metric Dimension} parameterized by the distance to clique does not admit a polynomial kernel unless $\NP \subseteq \coNP/poly$.
\end{theorem}

\begin{proof}
We slightly modify the reduction given in the proof of Theorem~\ref{polyker}: 
to the previously constructed graph $G$ in the proof of Theorem~\ref{polyker}, 
we simply add edges so that the vertices of $C_1,\dots,C_m$ induce a clique $K$ on $2m$ vertices.
Then the exact same proof as that of Theorem~\ref{polyker} still applies here since all of the distances mentioned in the proof of Theorem~\ref{polyker} remain the same in this construction.

Finally, it is easy to see that the distance to a clique of $G$ is at most $6n+3\alpha+3$ 
since deleting every vertex in $G$ except for the vertices of $K$ results in a clique.
Thus, the existence of a polynomial kernel for {\sc Metric Dimension} parameterized by the distance to clique would contradict the fact that there is no polynomial kernel for {\sc SAT} parameterized by the number of its variables,
which concludes the proof.
\end{proof}

